A Review of Software-Defined WLANs: Architectures and Central Control Mechanisms

The significant growth in the number of WiFi-enabled devices as well as the increase in the traffic conveyed through wireless local area networks (WLANs) necessitate the adoption of new network control mechanisms. Specifically, dense deployment of access points, client mobility, and emerging QoS demands bring about challenges that cannot be effectively addressed by distributed mechanisms. Recent studies show that software-defined WLANs (SDWLANs) simplify network control, improve QoS provisioning, and lower the deployment cost of new network control mechanisms. In this paper, we present an overview of SDWLAN architectures and provide a qualitative comparison in terms of features such as programmability and virtualization. In addition, we classify and investigate the two important classes of centralized network control mechanisms: (i) association control (AsC) and (ii) channel assignment (ChA). We study the basic ideas employed by these mechanisms, and in particular, we focus on the metrics utilized and the problem formulation techniques proposed. We present a comparison of these mechanisms and identify open research problems.

==> CA_Table-old.tex <==



%TABLE CA
\begin{table*}
	\centering
	\scriptsize
	\caption{Comparison of Channel Assignment (ChA) Mechanisms}
	\label{CA-table} 
	\def\arraystretch{1}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
		\Xhline{3\arrayrulewidth}
		%	\textbf{Ref.} & \multicolumn{2}{|c|}{OneTwoThree} & \multicolumn{2}{|c|}{OneTwoThree}&\textbf{Channels} & \textbf{Dynamic/Static} & \textbf{\multicolumn{2}{|c|}{OneTwoThree}}\\ \Xhline{3\arrayrulewidth}
		%		
		\multirow{2}{*}{Mechanism}&\multirow{2}{*}{\textbf{Client-Aware}}& \multicolumn{2}{c|}{Traffic-Aware}& \multicolumn{2}{c|}{Standards $\&$ Channels} & \multirow{2}{*}{\textbf{Dynamic}}&  \multicolumn{2}{c|}{Performance Evaluation}\\ \cline{3-6}\cline{8-9}
		
		&& \textbf{Downlink}& \textbf{Uplink}& \textbf{Standard} & \textbf{Partially Overlapping} & & \textbf{Simulation} & \textbf{Testbed}\\ \Xhline{3\arrayrulewidth}
		%1
		WCCA \cite{Wcolor-2005} &$\times$&$\times$&$\times$&802.11b&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$\\\hline
		%2
	    CDCA \cite{J-DCA-LB-2006}&$\checkmark$&$\times$&$\times$&802.11b&$\times$&$\checkmark$&$\checkmark$&$\checkmark$\\\hline
		%3
		%4
		%
		%		
		FPLN \cite{CAPWAP-based-CA-11}&$\times$&$\times$&$\times$&802.11b&$\checkmark$&$\times$&$\checkmark$&$\checkmark$\\\hline					
		%		
		%6
		% jCI \cite{DCA-2016-1}&$\checkmark$&$\checkmark$&$\times$&802.11b&$\times$&$\checkmark$&$\checkmark$&$\checkmark$\\\hline
		%
		%cloudmac-2013
		CloudMAC \cite{CloudMAC}&$\times$&$\times$&$\times$&802.11a/b/g/n&$\checkmark$&$\checkmark$&$\times$&$\checkmark$\\\hline		
		%		
		%Odin 2014
		Odin \cite{Odin2}&$\times$&$\times$&$\times$&802.11a/b/g/n&$\checkmark$&$\checkmark$&$\times$&$\checkmark$\\\hline				
		%		
		% -PCA 2015
		PCA \cite{802.11ac-PCA}&$\times$&$\times$&$\times$&802.11ac&$\times$&$\checkmark$&$\checkmark$&$\times$\\\hline		
		%
		EMPOWER2 \cite{Primitives}&$\times$&$\times$&$\times$&802.11a/b/g/n/ac&$\times$&$\checkmark$&$\times$&$\checkmark$\\\hline		
		%
		% -DCA-2 2016
		Wi5CA \cite{DCA-2}&$\times$&$\times$&$\times$&802.11b/g&$\times$&$\checkmark$&$\checkmark$&$\times$		 \\\hline
		%
		APCA \cite{J-AP-DCA-2006}&$\checkmark$&$\times$&$\checkmark$&802.11b&$\times$&$\times$&$\checkmark$&$\times$\\\hline		
		%		
		TACA \cite{Traffic-aware-CA-2007}&$\checkmark$&$\checkmark$&$\checkmark$&802.11b/g&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$\\\hline
		%		
		VDTCA \cite{Measurement-CA-WCNC-10}&$\checkmark$&$\checkmark$&$\checkmark$&802.11a/g&$\times$&$\checkmark$&$\times$&$\checkmark$\\\hline					
		%
		CUWN \cite{Cisco}&$\checkmark$&$\checkmark$&$\checkmark$&802.11a/b/g/n/ac&$\checkmark$&$\checkmark$&$\times$&$\times$\\\hline					
		%
		CAFA \cite{CA-F-WCNC-11}&$\checkmark$&$\checkmark$&$\checkmark$&802.11b&$\checkmark$&$\times$&$\checkmark$&$\times$ \\\hline
		%		
		TFACA \cite{CA-VTC-14}&$\times$&$\checkmark$&$\times$&802.11g&$\times$&$\times$&$\checkmark$&$\checkmark$\\\hline		
		%		
		FBWA \cite{CA-BW-VTC-14}&$\checkmark$&$\checkmark$&$\times$&802.11a/n/ac&$\times$&$\times$&$\checkmark$&$\times$\\\hline		
		%		
		NATCA \cite{DCA-residential-2015}&$\times$&$\checkmark$&$\times$&802.11g&$\times$&$\checkmark$&$\checkmark$&$\times$ 
		%\cite{Ch-usage-based-2016}&$\times$&$\times$&$\times$&$\times$&$\times$&$\times$&\\\hline		
		%
		%
		\\\Xhline{3\arrayrulewidth}
	\end{tabular}
\end{table*}

==> distributedMethods.tex <==
%\textcolor{blue}{
%\section{Summary of the studied papers}
%}
%\subsection{\textbf{\cite{VOID}}}
%\subsubsection{\textcolor{blue}{General useful information and challenges section of introduction}}
%The state-of-the-art approach to estimate interference relationships:
%\begin{itemize}
%\item Take the network temporarily offline (profile the network)
%\item Inject synthetic traffic for interference measurements 
%	\begin{itemize}
%	\item Sending unicast or broadcast packets and recording the information such as signal strength (RSSI) and packet delivery ratios (PDR).
%	\end{itemize}
%\item Use the measurements to seed various interference models to predict network performance at run-time\\
%\end{itemize}
%The advantage of the above approaches: produce \textbf{accurate static interference maps}\newline\\
%The drawbacks:
%\begin{itemize}
%\item it can be difficult or impossible for an administrator to gain control
%of all the wireless devices and take the network completely offline for measurement.
%\item the interference map may change over time, requiring these measurements to be taken periodically to capture these changes.
%\item network profiling is quite time consuming, requiring a few hours for a moderate-size network consisting of only 20 nodes.
%\item the drawback of the last proposed methods (using conflict tables, micro-probing or CTS-to-self packets)
%	\begin{itemize}
%		\item driver and protocol modification
%		\item cooperation from both APs and mobile clients
%	\end{itemize}
%\end{itemize}
%\subsubsection{\textcolor{blue}{Survey section}}
%\begin{itemize}
%\item (14,16,17,18,19): offline interference measurements
%\item (14,18,19): interference models (estimate interference relationships)
%\item (14): 802.11 state machine
%\item (18): Markov chain
%\item (19): RSSI/PDR
%\end{itemize}
%
%Interference handling techniques:
%\begin{itemize}
%\item (6,9): power adaptation
%\item (6,9,11): channel hopping
%\item (10): throttling at central routers
%\item (7,13): traffic scheduling
%\item (20]: ...
%\item (21): conflict graphs/maps and exchanging them among senders
%\item (5): micro-probing 
%\end{itemize}
%(22): Emulab wireless testbed\\
%\subsubsection{\textcolor{blue}{Simulation platform}}
%Emulab wireless testbed \\
%
%\textit{Brian White, Jay Lepreau, Leigh Stoller, Robert Ricci, Shashi Guruprasad, Mac Newbold, Mike Hibler, Chad Barb, and Abhijeet Joglekar. An integrated experimental environment for distributed systems and networks. In OSDI ’02}
%
%\subsection{\textbf{\cite{Mitigation-1}}}
%\subsubsection{\textcolor{blue}{General useful information and challenges section of introduction}}
%.\\
%Centralization:
%\begin{itemize}
%\item Control plane: feasible and easy
%\item \textbf{Data plane: complicated in high density WLANs (many APs)}\\
%\end{itemize}
%
%Two main approaches to mitigate the interference:
%\begin{itemize}
%\item Channel access management $\Rightarrow$ is not sufficient in dense AP deployments
%\item MAC contention strategy $\Rightarrow$ more important in dense WLANs
%	\begin{itemize}
%	\item Distributed mechanisms: ex. random access (DCF)
%		\begin{itemize}
%		\item simple and robust in practice
%		\item not require significant coordination between competing transmitters
%		\item \textbf{under-utilization}: it uses \textit{time} to resolve contention
%		\end{itemize}
%	\item Centralized mechanisms: ex. scheduled access
%		\begin{itemize}
%		\item if the traffic pattern at different nodes is \textit{regular} and \textit{predictable} 
%		\item $\Rightarrow$ it is possible to pre-compute an optimal transmission schedule
%		\item $\Rightarrow$ Under such \textit{predictability assumptions}, scheduling based approaches can outperform random access approaches.
%		\end{itemize}
%	\end{itemize}
%\end{itemize}
%
%\subsubsection{\textcolor{blue}{Main contribution of paper}}
%\begin{itemize}
%\item a general framework for designing efficient
%channel access mechanisms for enterprise WLANs $\Rightarrow$ more informed use of the wireless medium.
%\item significant centralized scheduling component
%\item limited amount of randomized contention
%\item named \textbf{speculative scheduling}
%\item no change the behavior of the underlying 802.11 MAC standard
%\end{itemize}
%
%key properties of channel contention framework:
%\begin{itemize}
%\item exact knowledge of a significant fraction ($80\%$) of traffic
%\item central entity $\Rightarrow$ co-located with the edge router of the WLAN
%\item two-stage hierarchy
%	\begin{itemize}
%	\item AP-level decisions $\Rightarrow$ a bounded amount of uncertainty at the central scheduler that is managed through speculation. 
%	\item feedback from the APs to central controller can be used to continually refine the scheduler’s global view and mitigate some of the uncertainty in future
%decisions.
%	\end{itemize}
%\item flexible design of scheduling policy: based on throughput, fairness, application-specific prioritization (Voice over WiFi)
%\item not require 802.11 clients to be aware of
%	\begin{itemize}
%	\item the new scheduling techniques
%	\item the existence of a central scheduler
%	\end{itemize}
%\item multi-AP association\\
%\end{itemize}
%
%\subsubsection{\textcolor{blue}{Details of mechanism}}
%\begin{itemize}
%\item compute the conflict graph periodically
%	\begin{itemize}
%	\item vertices: AP-client links
%	\item edge: if the corresponding links cannot be simultaneously active.
%		\begin{itemize}
%		\item AP-AP and client-client conflicts $\Rightarrow$ richer conflict graph (ref. [2])
%		\end{itemize}	
%	\end{itemize}
%\item compute a directed acyclic graph (DAG): presents the scheduling in order to transmit packets 
%\end{itemize}
%
%\subsubsection{\textcolor{blue}{Implementation}}
%.\\
%Two sub-systems:
%\begin{enumerate}
%\item conflict graph constructor (in the control plane)
%\item centralized scheduler (in the data plane)\\
%\end{enumerate}
%
%Both sub-systems run on a \textit{controller}, which is a standard desktop PC.
%
%\begin{itemize}
%\item The controller is connected to 30 custom-built APs using a 100 Mbps Ethernet switch.
%\item Each AP is built from a Soekris 4826 single-board computer node (ref. [1])
%	\begin{itemize}
%	\item running the 2.6.16.19 Linux kernel
%	\item equipped with an Intel 2915ABG mini-PCI wireless adapter
%	\end{itemize}
%\item The APs are deployed on five floors of an academic office building.
%\end{itemize}
%
%\subsubsection{\textcolor{blue}{Survey section}}
%\begin{itemize}
%\item (5,8,10): scheduling strategies 
%	\begin{itemize}
%	\item infer and learn traffic patterns along arbitrary single/multihop paths.
%	\item not use any centralized entity	
%	\end{itemize}
%\item (5,10): simple extensions to 802.11 standards
%\end{itemize}
%
%\subsection{\textbf{\cite{Mitigation-2}}}
%\subsubsection{\textcolor{blue}{Abstract}}
%\begin{itemize}
%\item a framework for interference mitigation
%in multi-BSS infrastructure 802.11 WLANs
%	\begin{itemize}
%	\item based on Access Point (AP) Coordination	
%	\end{itemize}
%\item negotiation among BSSs and switch from 802.11 CSMA/CA to a time-slotted mechanism if there is a 
%	\begin{itemize}
%	\item QoS degradation due to high interference
%	\end{itemize}	
%\item performance objective:
%	\begin{itemize}
%	\item utilize the bandwidth
%	\item improve the fairness among WLAN users
%	\end{itemize}	 
%\end{itemize}
%
%\subsubsection{\textcolor{blue}{General useful information and challenges section of introduction}}
%\begin{itemize}
%\item Channel assignment policies have a
%limited improvement potential especially under high load (multiple interfering BSSs).
%\item The 802.11e standard (enhanced to
%support QoS with multimedia) coordinates channel access within \textit{a BSS}.
%	\begin{itemize}
%	\item not address the problem of overlapping BSSs/cells that use the same channel.
%	\item no mechanism beyond CSMA/CA to
%coordinate the channel access across BSSs
%	\item BSSs operate asynchronously and independently
%	\end{itemize}
%\end{itemize}
%
%\subsubsection{\textcolor{blue}{Survey section}}
%\begin{itemize}
%\item (4): a managed WiFi system to support QoS in 802.11 WLANs with multiple BSSs
%	\begin{itemize}
%	\item \textit{Inter-AP coordination} to allow overlapping BSSs coordinate their operation during up-link transmissions of the \textit{Point Coordination Function (PCF)} modus so as to improve \textit{fairness among STAs}.
%	\item Weaknesses
%		\begin{enumerate}
%		\item purely attenuation-based  propagation model which is not the case in practice due to fading. 
%		\item the PCF modus is not supported by most IEEE 802.11-compliant products  
%		\item the BSS-based scheduling does not efficiently utilize the wireless bandwidth since it does not exploit exposed nodes within interfering BSSs which can simultaneously send their packets.		
%		\end{enumerate}
%	\end{itemize}
%\end{itemize}
%
%\subsubsection{\textcolor{blue}{Main idea}}
%\begin{itemize}
%\item The 802.11 CSMA/CA channel access scheme
%provides 
%	\begin{itemize}
%	\item \underline{best effort} service $\Rightarrow$ easy to implement, not need synchronization among contending nodes, works well at low traffic load  
%	\item At increased traffic levels
%		\begin{itemize}
%		\item interference $\uparrow$ \ $\Rightarrow$ frequent collisions, contention 	and retransmissions $\uparrow$
%	\end{itemize}
%	
%	\end{itemize}
%
%
%\item On the other hand, a collision-free channel access scheme, such as a \underline{time slotted access scheme}
%\begin{itemize}
%\item performs better than the CSMA/CA
%	\begin{itemize}
%	\item at high traffic loads
%	\end{itemize}
%\end{itemize}
%\end{itemize}
%
%$\Rightarrow$ A combination of above approaches is the main idea of this paper.
%
%\subsubsection{\textcolor{blue}{Simulation platform}}
%The NCTUns simulation package (\url{http://nsl.csie.nctu.edu.tw/nctuns.html})
%
%\subsubsection{\textcolor{blue}{Real implementation platform}}
%\begin{itemize}
%\item Two APs and five stationary STAs
%\item The APs are WLAN adapters from \underline{Atheros} configured in the
%master mode (AP mode) through \underline{the MADWIFI driver}.
%\item APs are connected via an Ethernet Switch.
%\item Over the ethernet connection, a \underline{master program} runs on one AP and  \underline{synchronizes both APs}.
%\end{itemize}
%
%\subsection{\textbf{\cite{optimal-design} valuable paper to read in detail!}}
%\subsubsection{\textcolor{blue}{Abstract}}
%\begin{itemize}
%\item high throughput performance $\Leftarrow$ deployment of a high density of Access Points
%	\begin{itemize}
%	\item $\Rightarrow$ additional interference
%	\end{itemize}
%\item the reaction of CSMA/CA protocol to interference 
%    \begin{itemize}
%    \item unnecessarily \underline{conservative} in high density environments
%	\end{itemize}     
%\item recommendations on \textbf{optimum dimensioning of high density networks}
%\item recommendations on \textbf{optimum tuning of the MAC parameters}
%\item results
%	\begin{enumerate}
%	\item 802.11a $\Rightarrow$ noise-dominated
%	\item 802.11g $\Rightarrow$ interference-dominated
%	\item MAC parameter tuning 
%		\begin{itemize}
%		\item limited benefit in properly planned 802.11a networks
%		\item substantial throughput improvements in 802.11g networks
%		\end{itemize}
%	\end{enumerate}
%\item an algorithm for the optimal tuning of MAC parameters in unstructured high density
%environments
%	\begin{itemize}
%	\item  260$\%$ improvement in network throughput	
%	\end{itemize}
%\end{itemize}
%\subsubsection{\textcolor{blue}{General useful information and challenges section of introduction}}
%\begin{itemize}
%\item small CCA threshold $\Rightarrow$ lower interference, lower throughput (reduced spatial reuse) 
%	\begin{itemize}
%	\item (2,3,4,5) papers focused on this issue
%	\end{itemize}
%\item the problem considered in this paper: optimal design and tuning of high density WiFi networks 
%	\begin{itemize}
%	\item at the minimum number of APs
%	\item best throughput performance to users
%	\end{itemize}
%	
%\item A single 802.11a/g AP
%	\begin{itemize}
%	\item coverage up to 100m at a data rate of 6 Mbps
%	\item in the presence of multiple users and time-varying wireless conditions\newline
%	$\Rightarrow$
%	actual throughput on the cell boundary may be \underline{much lower than 6 Mbps}\newline
%	$\Rightarrow$
%	deploy multiple APs over the region\newline
%	$\Rightarrow$
%	high density WLANs (cell radius of 20m to 50m) and interference plays a key role
%	\end{itemize}
%\item interference mitigation in cellular networks 
%	\begin{itemize}
%	\item per-user power control
%	\end{itemize}
%\item interference mitigation in WLANs
%	\begin{itemize}
%	\item based on the MAC protocol
%	\end{itemize}
%\item considering the following factors (In contrast
%to previous works (2,3,4,5): only MAC tuning)
%	\begin{itemize}
%	\item AP density
%	\item available number of orthogonal channels
%	\item different modulation and coding schemes
%	\item noise power
%	\item $SINR=\frac{S_R}{S_N+S_I}$
%	\item AP density $\uparrow$ $\Rightarrow$ $S_R\uparrow$
%	\item AP density $\uparrow$ $\Rightarrow$ $S_I\uparrow$
%	\item SINR $\uparrow$ $\Rightarrow$ data rate (throughput) $\uparrow$
%	\end{itemize}
%\item Identifying the operating-regime $\Rightarrow$ prime importance	
%	\begin{itemize}
%	\item noise-dominated network
%		\begin{itemize}
%		\item carrier sensing: almost \underline{no role} 
%		\item \textcolor{blue}{802.11a $\Rightarrow$ \textbf{12} orthogonal channels} 
%		\end{itemize}
%	\item interference-dominated network
%		\begin{itemize}
%		\item carrier sensing: \underline{pivotal role}
%		\item \textcolor{blue}{802.11g $\Rightarrow$ \textbf{3} orthogonal channels}
%		\end{itemize}		
%	\end{itemize}
%$\Rightarrow$ in determining the network throughput.	
%\item results:
%	\begin{itemize}
%	\item using the highest data rates $\Rightarrow$ may not be optimum from the overall network capacity perspective (in dense WLANs)		
%	\item based on the analytical results $\Rightarrow$ a \textcolor{blue}{CCA adaptation algorithm} $\Rightarrow$ mitigate the interference
%		\begin{itemize}
%		\item 2D and 3D environments
%		\item irrespective of the physical layer employed
%		\item irrespective of the efficiency of the frequency selection mechanism
%		\item no assumptions about the operating regime of the network
%		\item throughput $\Leftrightarrow$ interference
%		\item throughput improvement
%			\begin{itemize}
%			\item 260$\%$: compared to default MAC
%			\item 30$\%$: compared to ECHOS (ref. 18)
%			\end{itemize}
%		\end{itemize}
%	\end{itemize}
%\end{itemize}
%
%\subsubsection{\textcolor{blue}{Main ideas}}
%. \\
%Network design choices in order to avoid the adverse effect of interference in high density WLANs:
%\begin{enumerate}[i)]
%\item identification of PHY technology (g or a)
%\item choice of AP density
%\item channel selection (minimum contention)
%\item tuning of MAC parameters
%\end{enumerate}

% use section* for acknowledgement
%%%%%%% \section*{Acknowledgment}


%The authors would like to thank...

% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://www.ctan.org/tex-archive/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)


==> references111.tex <==

\begin{thebibliography}{1}

\bibitem{NextGen-WiFi-Survey-2016} H. A. Omar, K. Abboud, N. Cheng, K. R. Malekshan, A. T. Gamage, and W. Zhuang, "A Survey on High Efficiency Wireless Local Area Networks: Next Generation WiFi," IEEE Communications Surveys Tutorials, vol. 18, no. 4, pp. 2315-2344, 2016.

\bibitem{WiFi-Devices} IC Insights. n.d. "Global Wi-Fi enabled equipment shipments from 2012 to 2017 (in billion units)". Statista. Available: https://www.statista.com/statistics/282512/global-wi-fi-enabled-equipment-shipments/. 

\bibitem{Cisco-statistics} "Cisco Visual Networking Index: Global Mobile Data Traffic Forecast Update, 2015–-2020 White Paper," Cisco. Available: http://www.cisco.com/c/en/us/solutions/collateral/service-provider/visual-networking-index-vni/mobile-white-paper-c11-520862.html.

\bibitem{Offloading} K. Lee, J. Lee, Y. Yi, I. Rhee, and S. Chong, "Mobile Data Offloading: How Much Can WiFi Deliver?," IEEE/ACM Transactions on Networking, vol. 21, no. 2, pp. 536-550, Apr. 2013.

\bibitem{Offloading-survey-2016} Y. He, M. Chen, B. Ge, and M. Guizani, "On WiFi Offloading in Heterogeneous Networks: Various Incentives and Trade-Off Strategies," IEEE Communications Surveys Tutorials, vol. 18, no. 4, pp. 2345–2385, 2016.

\bibitem{Experimenting802.11} P. Serrano, P. Salvador, V. Mancuso, and Y. Grunenberger, “Experimenting with commodity 802.11 hardware: Overview and future directions,” IEEE Commun. Surv. Tutorials, vol. 17, no. 2, pp. 671–699, 2015.

\bibitem{NGwlans-survey-2016} B. Bellalta, L. Bononi, R. Bruno, and A. Kassler, "Next generation IEEE 802.11 Wireless Local Area Networks: Current status, future directions and open challenges," Computer Communications, vol. 75, pp. 1-25, Feb. 2016.



\bibitem{DenseWLAN1} V. P. Mhatre, K. Papagiannaki, and F. Baccelli, “Interference Mitigation Through Power Control in High Density 802.11 WLANs,” 26th IEEE International Conference on Computer Communications (INFOCOM). pp. 535–543, 2007.


\bibitem{DenseWLAN2} I. Broustis, K. Papagiannaki, S. V. Krishnamurthy, M. Faloutsos, and V. P. Mhatre, “Measurement-driven guidelines for 802.11 WLAN design,” IEEE/ACM Trans. Netw., vol. 18, no. 3, pp. 722–735, 2010.

\bibitem{UltraDense} M. Kamel, W. Hamouda, and A. Youssef, “Ultra-Dense Networks: A Survey,” IEEE Commun. Surv. Tutorials, vol. 18, no. 4, pp. 2522–2545, 2016.

\bibitem{BIGAP} A. Zubow, S. Zehl, and A. Wolisz, “BIGAP — Seamless handover in high performance enterprise IEEE 802.11 networks,” in IEEE/IFIP Network Operations and Management Symposium (NOMS), 2016, pp. 445–453.

\bibitem{AmorFi} R. K Sheshadri, M. Y. Arslan, K. Sundaresan, S. Rangarajan, and D. Koutsonikolas, “AmorFi: Amorphous WiFi Networks for High-density Deployments,” in Proceedings of the 12th International on Conference on emerging Networking EXperiments and Technologies - CoNEXT ’16, 2016, pp. 161–175.


\bibitem{QoS-WLANs} J. Choi and K. G. Shin, "QoS provisioning for large-scale multi-ap WLANs," Ad Hoc Networks, vol. 10, no. 2, pp. 174-185, Mar. 2012.

\bibitem{NOX} N. Gude, T. Koponen, J. Pettit, B. Pfaff, M. Casado, N. McKeown, and S. Shenker, “NOX: towards an operating system for networks,” SIGCOMM Comput. Commun. Rev., vol. 38, no. 3, pp. 105–110, 2008.

\bibitem{OpenFlow} N. McKeown, T. Anderson, H. Balakrishnan, G. Parulkar, L. Peterson, J. Rexford, S. Shenker, and J. Turner, “OpenFlow: Enabling Innovation in Campus Networks,” ACM SIGCOMM Comput. Commun. Rev., vol. 38, no. 2, p. 69, 2008.

\bibitem{ONF} Open Networking Foundation. Available: https://www.opennetworking.org/

\bibitem{SDN1} Y. Jarraya, T. Madi, and M. Debbabi, "A Survey and a Layered Taxonomy of Software-Defined Networking," IEEE Communications Surveys Tutorials, vol. 16, no. 4, pp. 1955-1980, 2014.

\bibitem{SDN2} D. B. Rawat and S. R. Reddy, "Software Defined Networking Architecture, Security and Energy Efficiency: A Survey," IEEE Communications Surveys Tutorials, vol. PP, no. 99, pp. 1–1, 2016.

\bibitem{wSDN1} I. T. Haque and N. Abu-Ghazaleh, "Wireless Software Defined Networking: A Survey and Taxonomy," IEEE Communications Surveys Tutorials, vol. 18, no. 4, pp. 2713–2737, 2016.

\bibitem{mSDN2} T. Chen, M. Matinmikko, X. Chen, X. Zhou, and P. Ahokangas, "Software defined mobile networks: concept, survey, and research directions," IEEE Communications Magazine, vol. 53, no. 11, pp. 126-133, Nov. 2015.

\bibitem{Primitives} R. Riggio, M. K. Marina, J. Schulz-Zander, S. Kuklinski, and T. Rasheed, "Programming Abstractions for Software-Defined Wireless Networks," IEEE Transactions on Network and Service Management, vol. 12, no. 2, pp. 146-162, Jun. 2015.



%\bibitem{[2]} B. A. A. Nunes, M. Mendonca, X. N. Nguyen, K. Obraczka, and T. Turletti, “A Survey of Software-Defined Networking: Past, Present, and Future of Programmable Networks,” IEEE Communications Surveys Tutorials, vol. 16, no. 3, pp. 1617–1634, Third 2014.
%[3]F. Hu, Q. Hao, and K. Bao, “A Survey on Software-Defined Network and OpenFlow: From Concept to Implementation,” IEEE Communications Surveys Tutorials, vol. 16, no. 4, pp. 2181–2206, Fourthquarter 2014.
%[4]W. Xia, Y. Wen, C. H. Foh, D. Niyato, and H. Xie, “A Survey on Software-Defined Networking,” IEEE Communications Surveys Tutorials, vol. 17, no. 1, pp. 27–51, Firstquarter 2015.
%[5]Y. Li and M. Chen, “Software-Defined Network Function Virtualization: A Survey,” IEEE Access, vol. 3, pp. 2542–2553, 2015.




%% Association

%% TPC 
%\bibitem{TPC1} V. P. Mhatre, K. Papagiannaki, and F. Baccelli, "Interference Mitigation Through Power Control in High Density 802.11 WLANs," in IEEE INFOCOM 2007 - 26th IEEE International Conference on Computer Communications, 2007, pp. 535-543.
%
%\bibitem{TPC2} H. Ma, J. Zhu, S. Roy, and S. Y. Shin, "Joint transmit power and physical carrier sensing adaptation based on loss differentiation for high density IEEE 802.11 WLAN," Computer Networks, vol. 52, no. 9, pp. 1703-1720, Jun. 2008.
%
%\bibitem{TPC3}J. Chen, S. Olafsson, Y. Yang, and X. Gu, "Joint Distributed Transmit Power Control and Dynamic Channel Allocation for Scalable WLANs," in 2009 IEEE Wireless Communications and Networking Conference, 2009, pp. 1-6.
%
%\bibitem{TPC4} W. Li, Y. Cui, X. Cheng, M. A. Al-Rodhaan, and A. Al-Dhelaan, "Achieving Proportional Fairness via AP Power Control in Multi-Rate WLANs," IEEE Transactions on Wireless Communications (WCNC), vol. 10, no. 11, pp. 3784-3792, Nov. 2011.
%
%\bibitem{TPC5} Y. Wu, Y. Sun, Y. Ji, J. Mao, and Y. Liu, "A joint channel allocation and power control scheme for interference mitigation in high-density WLANs," in 2013 15th IEEE International Conference on Communication Technology, 2013, pp. 98-103.
%
%\bibitem{TPC6} S. Kamiya, K. Nagashima, K. Yamamoto, T. Nishio, M. Morikura, and T. Sugihara, "Joint range adjustment and channel assignment for overlap mitigation in dense WLANs," in 2015 IEEE 26th Annual International Symposium on Personal, Indoor, and Mobile Radio Communications (PIMRC), 2015, pp. 1974-1979.

\bibitem{APdensity} K. Sui et al., "Understanding the Impact of AP Density on WiFi Performance Through Real-World Deployment," in 2016 IEEE International Symposium on Local and Metropolitan Area Networks (LANMAN), 2016, pp. 1-6.

\bibitem{SDN-IoT-survey} K. Sood, S. Yu, and Y. Xiang, "Software-Defined Wireless Networking Opportunities and Challenges for Internet-of-Things: A Review," IEEE Internet of Things Journal, vol. 3, no. 4, pp. 453-463, Aug. 2016.

%%%% Survey Papers

\bibitem{S9-Channel} A. Baid and D. Raychaudhuri, "Understanding channel selection dynamics in dense Wi-Fi networks," IEEE Communications Magazine, vol. 53, no. 1, pp. 110-117, Jan. 2015.

\bibitem{802.11aa} IEEE Std 802.11aa-2012: Specific requirements Part11: Wireless LAN Medium Access Control (MAC) and Physical Layer (PHY) Specifications Amendment2: MAC Enhancements for Robust Audio Video Streaming, 2012.

\bibitem{802.11ac} IEEE Std P802.11ac-2013: Part11: Wireless LAN Medium Access Control (MAC) and Physical Layer (PHY) specifications: Enhancements for Very High Throughput for Operation in Bands below 6GHz, 2013.

\bibitem{802.11af} IEEE802.11af-2013: Local and metropolitan area networks Part11: Wireless LAN Medium Access Control (MAC) and Physical Layer (PHY) Specifications Amendment5: Television White Spaces (TVWS) Operation, 2013.

\bibitem{802.11ah} IEEE P802.11ah/D10.0, "IEEE Approved Draft Standard for Information Technology-Telecommunications and Information Exchange Between Systems-Local and Metropolitan Area Networks-Specific Requirements-Part 11: Wireless LAN Medium Access Control (MAC) and Physical Layer (PHY) Specifications: Amendment 2: Sub 1 GHz License Exempt Operation," 2016.

\bibitem{S1-energy-MAC} S.-L. Tsao and C.-H. Huang, “A survey of energy efficient MAC protocols for IEEE 802.11 WLAN,” Computer Communications, vol. 34, no. 1, pp. 54–67, Jan. 2011.

\bibitem{S2-QoS} E. Charfi, L. Chaari, and L. Kamoun, "PHY/MAC Enhancements and QoS Mechanisms for Very High Throughput WLANs: A Survey," IEEE Communications Surveys Tutorials, vol. 15, no. 4, pp. 1714-1735, Fourth 2013.

\bibitem{S3-QoS} Q. Ni, L. Romdhani, and T. Turletti, “A survey of QoS enhancements for IEEE 802.11 wireless LAN,” Wirel. Commun. Mob. Comput., vol. 4, no. 5, pp. 547–566, Aug. 2004.

\bibitem{S4-QoS} J. Choi and K. G. Shin, "QoS provisioning for large-scale multi-ap WLANs," Ad Hoc Networks, vol. 10, no. 2, pp. 174-185, Mar. 2012.

\bibitem{S5-LB} L. H. Yen, T. T. Yeh, and K. H. Chi, "Load Balancing in IEEE 802.11 Networks," IEEE Internet Computing, vol. 13, no. 1, pp. 56-64, Jan. 2009.

\bibitem{S6-Intf} M. Hoyhtya et al., "Spectrum Occupancy Measurements: A Survey and Use of Interference Maps," IEEE Communications Surveys Tutorials, vol. 18, no. 4, pp. 2386-2414, 2016.

\bibitem{S7-ax} B. Bellalta, "IEEE 802.11ax: High-efficiency WLANs," IEEE Wireless Communications, vol. 23, no. 1, pp. 38-46, Feb. 2016.


\bibitem{largeScaleMeas} S. Biswas, J. Bicket, E. Wong, R. Musaloiu-E, A. Bhartia, and D. Aguayo, “Large-scale Measurements of Wireless Network Behavior,” in Proceedings of the 2015 ACM Conference on Special Interest Group on Data Communication - SIGCOMM ’15, 2015, pp. 153–165.


\bibitem{SDNscalability} S. H. Yeganeh, A. Tootoonchian, and Y. Ganjali, “On scalability of software-defined networking,” IEEE Commun. Mag., vol. 51, no. 2, pp. 136–141, 2013.

\bibitem{SDNsurvey} I. T. Haque and N. Abu-ghazaleh, “Wireless Software Defined Networking: A Survey and Taxonomy,” IEEE Commun. Surv. Tutorials, vol. 18, no. 4, pp. 1–25, 2016.

\bibitem{SDNLang} C. Trois, M. D. D. Del Fabro, L. C. E. de Bona, and M. Martinello, “A Survey on SDN Programming Languages: Towards a Taxonomy,” IEEE Commun. Surv. Tutorials, vol. PP, no. 99, p. 1, 2016.

\bibitem{RSSIranging} A. Zanella, “Best Practice in RSS Measurements and Ranging,” IEEE Commun. Surv. Tutorials, vol. 18, no. 4, pp. 2662–2686, 2016.

\bibitem{decIntf} A. Kashyap, U. Paul, and S. R. Das, “Deconstructing Interference Relations in WiFi Networks,” in 7th Annual IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks (SECON), 2010, pp. 1–9.

\bibitem{smog} S. Gollakota, F. Adib, D. Katabi, and S. Seshan, “Clearing the RF Smog: Making 802.11 Robust to Cross-Technology Interference,” in Proceedings of the ACM SIGCOMM 2011 conference, 2011, p. 170.


\bibitem{Crowd} H. Ali-Ahmad, C. Cicconetti, A. de la Oliva, M. Draxler, R. Gupta, V. Mancuso, L. Roullet, and V. Sciancalepore, “CROWD: An SDN Approach for DenseNets,” in econd European Workshop on Software Defined Networks, 2013, pp. 25–31.
\bibitem{SDNcellular} L. E. Li, Z. M. Mao, and J. Rexford, “Toward Software-Defined Cellular Networks,” in European Workshop on Software Defined Networking, 2012, pp. 7–12.

\bibitem{FlashBack} A. Cidon, K. Nagaraj, S. Katti, and P. Viswanath, “Flashback: Decoupled Lightweight Wireless Control,” in Proceedings of the ACM SIGCOMM 2012 conference on Applications, technologies, architectures, and protocols for computer communication - SIGCOMM ’12, 2012, p. 223.

\bibitem{SplitAP} G. Bhanage, D. Vete, I. Seskar, and D. Raychaudhuri, “SplitAP: Leveraging Wireless Network Virtualization for Flexible Sharing of WLANs,” in IEEE Global Telecommunications Conference GLOBECOM, 2010, pp. 1–6.

\bibitem{ViFi} K. Guo, S. Sanadhya, and T. Woo, “ViFi: Virtualizing WLAN using commodity hardware,” in 9th ACM MobiCom Workshop on Mobility in the Evolving Internet Architecture, MobiArch 2014, 2014, vol. 18, no. 3, pp. 25–30.

%\bibitem{Ethane} M. Casado, M. J. Freedman, J. Pettit, J. Luo, N. McKeown, and S. Shenker, "Ethane: taking control of the enterprise," SIGCOMM Comput. Commun. Rev., vol. 37, no. 4, pp. 1-12, Aug. 2007.

\bibitem{DIRAC} P. Zerfos, G. Zhong, J. Cheng, H. Luo, S. Lu, and J. J.-R. Li, “DIRAC: A Software-based Wireless Router System,” in Proceedings of the 9th annual international conference on Mobile computing and networking - MobiCom ’03, 2003, p. 230.

\bibitem{DenseAP} R. Murty, J. Padhye, R. Chandra, A. Wolman, and B. Zill, "Designing high performance enterprise Wi-Fi networks," in Proceedings of the 5th USENIX Symposium on Networked Systems Design and Implementation, 2008.

\bibitem{Trantor} R. Murty, J. Padhye, A. Wolman, and M. Welsh, "An Architecture for Extensible Wireless LANs," in ACM Hotnets, pp. 79 - 84, 2008.

\bibitem{Dyson} R. Murty, J. Padhye, A. Wolman, and M. Welsh, "Dyson: An Architecture for Extensible Wireless LANs," in Proceedings of the 2010 USENIX conference on USENIX annual technical conference, 2010.

%\bibitem{CENTAUR} V. Shrivastava et al., "CENTAUR: Realizing the Full Potential of Centralized Wlans Through a Hybrid Data Path," in Proceedings of the 15th Annual International Conference on Mobile Computing and Networking, New York, NY, USA, 2009, pp. 297-308.

\bibitem{WLANlocalization} R. Chandra, J. Padhye, A. Wolman, and B. Zill, "A Location-Based Management System for Enterprise Wireless LANs". In NSDI, 2007.

\bibitem{LWAPP} R. Suri, N. Cam Winget, M. Williams, S. Hares, B. O'Hara, and S. Kelly, "Lightweight Access Point Protocol." [Online]. Available: https://tools.ietf.org/html/rfc5412.

\bibitem{CAPWAP} D. Stanley, P. Calhoun, and M. Montemurro, "Control And Provisioning of Wireless Access Points (CAPWAP) Protocol Specification." [Online]. Available: https://tools.ietf.org/html/rfc5415.

\bibitem{DTLS} N. Modadugu and E. Rescorla, "Datagram Transport Layer Security." [Online]. Available: https://tools.ietf.org/html/rfc4347.

\bibitem{Cisco} J. Smith, J. Woodhams, and R. Marg, Controller-Based Wireless LAN Fundamentals: An end-to-end reference guide to design, deploy, manage, and secure 802.11 wireless networks, Indianapolis, IN: Cisco Press, 2011.
\bibitem{CiscoRRM} Radio Resource Management under Unified Wireless Networks, Available: http://www.cisco.com/c/en/us/support/docs/wireless-mobility/wireless-lan-wlan/71113-rrm-new.html

\bibitem{Odin} L. Suresh, J. Schulz-Zander, R. Merz, A. Feldmann, and T. Vazao, "Towards Programmable Enterprise WLANS with Odin," in Proceedings of the First Workshop on Hot Topics in Software Defined Networks, 2012, pp. 115-120.

\bibitem{Odin2} J. Schulz-Zander, L. Suresh, N. Sarrar, A. Feldmann, T. Hühn, and R. Merz, “Programmatic Orchestration of WiFi Networks,” in USENIX Annual Technical Conference, 2014, pp. 347–358.

\bibitem{OdinThor} R. Riggio, C. Sengul, L. Suresh, J. Schulz–zander, and A. Feldmann, “Thor: Energy programmable WiFi networks,” in IEEE Conference on Computer Communications Workshops (INFOCOM WKSHPS), 2013, pp. 21–22.

\bibitem{OdinSource} “Odin Source.” [Online]. Available: http://sdn.inet.tu-berlin.de.

\bibitem{Blueprints} K.-K. Yap, R. Sherwood, M. Kobayashi, T.-Y. Huang, M. Chan, N. Handigol, N. McKeown, and G. Parulkar, “Blueprint for introducing innovation into wireless mobile networks,” in Proceedings of the second ACM SIGCOMM workshop on Virtualized infrastructure systems and architectures - VISA ’10, 2010, p. 25.

\bibitem{vBS} K. Nakauchi and Y. Shoji, “WiFi Network Virtualization to Control the Connectivity of a Target Service,” IEEE Trans. Netw. Serv. Manag., vol. 12, no. 2, pp. 308–319, Jun. 2015.

\bibitem{VAN} V. Sivaraman, T. Moors, H. Habibi Gharakheili, D. Ong, J. Matthews, and C. Russell, “Virtualizing the access network via open APIs,” in Proceedings of the ninth ACM conference on Emerging networking experiments and technologies - CoNEXT ’13, 2013, pp. 31–42.

\bibitem{CloudMAC} J. Vestin, P. Dely, A. Kassler, N. Bayer, H. Einsiedler, and C. Peylo, "CloudMAC: Towards Software Defined WLANs," ACM SIGMOBILE Mobile Computing and Communications Review, vol. 16, no. 4, pp. 42-45, Feb. 2013.
\bibitem{CloudMAC2} J. Vestin, P. Dely, A. Kassler, N. Bayer, H. Einsiedler, and C. Peylo, “CloudMAC- Towards Software Defined WLANs,” ACM SIGMOBILE Mob. Comput. Commun. Rev., vol. 16, no. 4, p. 42, Feb. 2013.

\bibitem{CloudMAC3} J. Vestin and A. Kassler, “QoS enabled WiFi MAC layer processing as an example of a NFV service,” in Proceedings of the 1st IEEE Conference on Network Softwarization (NetSoft), 2015, pp. 1–9.

\bibitem{capsulator} “Capsulator.” [Online]. Available: http://archive.openow.org/wk/index.php/Capsulator.
\bibitem{OpenWRT} “OpenWRT.” [Online]. Available: https://openwrt.org.
\bibitem{OpenvSwitch} “OpenvSwitch.” [Online]. Available: http://openvswitch.org.

\bibitem{BeHop} Y. Yiakoumis, M. Bansal, A. Covington, J. van Reijendam, S. Katti, and N. McKeown, "BeHop: A Testbed for Dense WiFi Networks," ACM SIGMOBILE Mobile Computing and Communications Review, vol. 18, no. 3, pp. 71-80, Jan. 2015.

\bibitem{OpenSDWN} J. Schulz-Zander, C. Mayer, B. Ciobotaru, S. Schmid, and A. Feldmann, "OpenSDWN: Programmatic Control over Home and Enterprise WiFi," in Proceedings of the 1st ACM SIGCOMM Symposium on Software Defined Networking Research, New York, NY, USA, 2015, p. 16:1-16:12.

\bibitem{SDWLAN} D. Zhao, M. Zhu, and M. Xu, "SDWLAN: A flexible architecture of enterprise WLAN for client-unaware fast AP handoff," in 2014 International Conference on Computing, Communication and Networking Technologies (ICCCNT), 2014, pp. 1-6.
\bibitem{SDWLAN2} D. Zhao, M. Zhu, and M. Xu, “Supporting ‘One Big AP’ illusion in enterprise WLAN: An SDN-based solution,” in Sixth International Conference on Wireless Communications and Signal Processing (WCSP), 2014, pp. 1–6.


\bibitem{EmPOWER} R. Riggio, T. Rasheed, and F. Granelli, "EmPOWER: A Testbed for Network Function Virtualization Research and Experimentation," in Future Networks and Services (SDN4FNS), 2013 IEEE SDN for, 2013, pp. 1-5.

\bibitem{EmPOWER-src} “EmPOWER.” [Online]. Available: http://empower.create-net.org/.


\bibitem{Ethanol} H. Moura, G. V. C. Bessa, M. A. M. Vieira, and D. F. Macedo, "Ethanol: Software defined networking for 802.11 Wireless Networks," in 2015 IFIP/IEEE International Symposium on Integrated Network Management (IM), 2015, pp. 388-396.

\bibitem{COAP} A. Patro and S. Banerjee, "COAP: A Software-Defined Approach for Home WLAN Management Through an Open API," SIGMOBILE Mob. Comput. Commun. Rev., vol. 18, no. 3, pp. 32-40, Jan. 2015.

\bibitem{Energino} Energino website, Available: http://www.energino-project.org.

\bibitem{AeroFlux} J. Schulz-Zander, N. Sarrar and S. Schmid, "AeroFlux: A Near-Sighted Controller Architecture for Software-Defined Wireless Networks", Open Networking Summit (ONS), 2014.  

\bibitem{AeroFlux2} J. Schulz-Zander, N. Sarrar, and S. Schmid, “Towards a scalable and near-sighted control plane architecture for WiFi SDNs,” in Proceedings of the third workshop on Hot topics in software defined networking - HotSDN ’14, 2014, pp. 217–218.



\bibitem{OpenRadio} M. Bansal, J. Mehlman, S. Katti, and P. Levis, “OpenRadio: A Programmable Wireless Dataplane,” in HotSDN, 2012, pp. 109–114.

\bibitem{Atomix} M. Bansal, A. Schulman, and S. Katti, “Atomix: A Framework for Deploying Signal Processing Applications on Wireless Infrastructure,” in 12th USENIX Symposium on Networked Systems Design and Implementation (NSDI 15), 2015, pp. 173–188.

\bibitem{Sora} K. Tan, H. Liu, J. Zhang, Y. Zhang, J. Fang, and G. M. Voelker, “Sora: High-Performance Software Radio Using General-Purpose Multi-Core Processors,” in Communications of the ACM, 2011, vol. 54, no. 1, p. 99.


\bibitem{hostapd} hostapd: IEEE 802.11 AP, IEEE 802.1X/WPA/WPA2/EAP/RADIUS Authenticator, Available: https://w1.fi/hostapd/

\bibitem{zerorpc} J. Petazzoni, “Build reliable, traceable, distributed systems with zeromq (zerorpc),” Available: http://pycon-2012-notes.readthedocs.org/en/latest/- dotcloud zerorpc.html

\bibitem{zeromq} iMatix Corporation, “Zmq - code connected,” Available: http://zeromq.org/.


\bibitem{Picasso} S. S. Hong, J. Mehlman, and S. Katti, “Picasso: Flexible RF and Spectrum Slicing,” in SIGCOMM Comput. Commun. Rev., 2012, vol. 42, no. 4, pp. 37–48.

\bibitem{OpenSketch} M. Yu, L. Jose, and R. Miao, “Software defined traffic measurement with opensketch,” in 10th USENIX Symposium on Networked Systems, 2013, pp. 29–42.

\bibitem{SpotFi} M. Kotaru, K. Joshi, D. Bharadia, and S. Katti, “SpotFi: Decimeter Level Localization Using WiFi,” in ACM SIGCOMM Computer Communication Review, 2015, vol. 45, no. 5, pp. 269–282.

\bibitem{Pantou} Pantou for OpenWRT, Available: https://www.sdxcentral.com/ projects/ pantou-openwrt/.

\bibitem{AEtherFlow} M. Yan, J. Casey, P. Shome, A. Sprintson, and A. Sutton, “$\AE$therFlow: Principled Wireless Support in SDN,” in IEEE 23rd International Conference on Network Protocols (ICNP), 2015, pp. 432–437.

\bibitem{ofsoftswitch} ofsoftswitch, Available: https://github.com/CPqD/ofsoftswitch13

%\bibitem{CROWD} H. Ali-Ahmad et al., "CROWD: An SDN Approach for DenseNets," in 2013 Second European Workshop on Software Defined Networks, 2013, pp. 25-31.
\bibitem{ResFi} S. Zehl, A. Zubow, M. Doring, and A. Wolisz, “ResFi: A secure framework for self organized Radio Resource Management in residential WiFi networks,” in IEEE 17th International Symposium on A World of Wireless, Mobile and Multimedia Networks (WoWMoM), 2016, pp. 1–11.
%\bibitem{SWAN} T. Lei, Z. Lu, X. Wen, X. Zhao, and L. Wang, "SWAN: An SDN based campus WLAN framework," in 2014 4th International Conference on Wireless Communications, Vehicular Technology, Information Theory and Aerospace Electronic Systems (VITAE), 2014, pp. 1-5.
%\bibitem{WiPCon} W. S. Kim, S. H. Chung, and J. Shi, "WiPCon: A Proxied Control Plane for Wireless Access Points in Software Defined Networks," in 2014 IEEE 17th International Conference on Computational Science and Engineering, 2014, pp. 923-929.

%\bibitem{OpenNet} M. C. Chan, C. Chen, J. X. Huang, T. Kuo, L. H. Yen, and C. C. Tseng, "OpenNet: A simulator for software-defined wireless local area network," in 2014 IEEE Wireless Communications and Networking Conference (WCNC), 2014, pp. 3332-3336.

%\bibitem{OneBigAP}D. Zhao, M. Zhu, and M. Xu, "Supporting One Big AP illusion in enterprise WLAN: An SDN-based solution," in 2014 Sixth International Conference on Wireless Communications and Signal Processing (WCSP), 2014, pp. 1-6.

\bibitem{Floodlight} Project floodlight. Available: http://www.projectfloodlight.org/floodlight.


\bibitem{OVS} Open vSwitch website, Available: http://openvswitch.org.

\bibitem{OpenCAPWAP} M. Bernaschi, F. Cacace, G. Iannello, M. Vellucci, and L. Vollero, "OpenCAPWAP: An open source CAPWAP implementation for the management and configuration of WiFi hot-spots," Computer Networks, vol. 53, no. 2, pp. 217-230, Feb. 2009.

\bibitem{LCCS} M. Achanta, "Method and Apparatus for Least Congested Channel Scan for Wireless Access Points," US Patent No. 20060072602, Apr. 2006.

\bibitem{Channel-assignment-survey-2010} S. Chieochan, E. Hossain, and J. Diamond, "Channel assignment schemes for infrastructure-based 802.11 WLANs: A survey," IEEE Communications Surveys Tutorials, vol. 12, no. 1, pp. 124-136, Firstquarter 2010.

\bibitem{DCA-G-1}M. Drieberg, F. C. Zheng, R. Ahmad, and S. Olafsson, "An Asynchronous Distributed Dynamic Channel Assignment Scheme for Dense WLANs," in 2008 IEEE International Conference on Communications, 2008, pp. 2507-2511.
\bibitem{DCA-G-2}X. Yue, C. F. Wong, and S. H. G. Chan, "CACAO: Distributed Client-Assisted Channel Assignment Optimization for Uncoordinated WLANs," IEEE Transactions on Parallel and Distributed Systems, vol. 22, no. 9, pp. 1433-1440, Sep. 2011.
\bibitem{DCA-G-3} K. Zhou, X. Jia, L. Xie, Y. Chang, and X. Tang, "Channel assignment for WLAN by considering overlapping channels in SINR interference model," in 2012 International Conference on Computing, Networking and Communications (ICNC), 2012, pp. 1005-1009.
\bibitem{DCA-G-4} H. Al-Rizzo, M. Haidar, R. Akl, and Y. Chan, "Enhanced Channel Assignment and Load Distribution in IEEE 802.11 WLANs," in 2007 IEEE International Conference on Signal Processing and Communications, 2007, pp. 768-771.

\bibitem{usagePatterns} M. Afanasyev, T. Chen, G. M. Voelker, and A. C. Snoeren, “Usage patterns in an urban WiFi network,” IEEE/ACM Trans. Netw., vol. 18, no. 5, pp. 1359–1372, 2010.

\bibitem{transOpp} D. Giustiniano, D. Malone, D. J. Leith, and K. Papagiannaki, “Measuring transmission opportunities in 802.11 links,” IEEE/ACM Trans. Netw., vol. 18, no. 5, pp. 1516–1529, 2010.

\bibitem{Wcolor-2005} A. Mishra, S. Banerjee, and W. Arbaugh, "Weighted Coloring Based Channel Assignment for WLANs," ACM SIGMOBILE Mobile Computing and Communications Review, vol. 9, no. 3, pp. 19-31, Jul. 2005.

\bibitem{J-DCA-LB-2006} A. Mishra, V. Brik, S. Banerjee, A. Srinivasan, and W. Arbaugh, "A Client-driven Approach for Channel Management in Wireless LANs," in Proc. 25th IEEE International Conference on Computer Communications (INFOCOM’06), 2006.

\bibitem{J-AP-DCA-2006} X. Ling and K. L. Yeung, "Joint access point placement and channel assignment for 802.11 wireless LANs," IEEE Transactions on Wireless Communications, vol. 5, no. 10, pp. 2705-2711, Oct. 2006.

\bibitem{Traffic-aware-CA-2007} E. Rozner, Y. Mehta, A. Akella, and L. Qiu, "Traffic-Aware Channel Assignment in Enterprise Wireless LANs," in 2007 IEEE International Conference on Network Protocols, 2007, pp. 133-143.

\bibitem{802.11ac-PCA} S. Jang and S. Bahk, "A Channel Allocation Algorithm for Reducing the Channel Sensing/Reserving Asymmetry in 802.11ac Networks," IEEE Transactions on Mobile Computing, vol. 14, no. 3, pp. 458-472, Mar. 2015.

\bibitem{DCA-2016-1} K. Lee, Y. Kim, S. Kim, J. Shin, S. Shin, and S. Chong, "Just-in-time WLANs: On-demand interference-managed WLAN infrastructures," in IEEE INFOCOM 2016 - The 35th Annual IEEE International Conference on Computer Communications, 2016, pp. 1-9.

\bibitem{DCA-2} M. Seyedebrahimi, F. Bouhafs, A. Raschellà, M. Mackay, and Q. Shi, "SDN-based channel assignment algorithm for interference management in dense Wi-Fi networks," in 2016 European Conference on Networks and Communications (EuCNC), 2016, pp. 128-132.

\bibitem{Wi-5} Wi-5Project(What to do With the Wi-Fi Wild West),t. Available: http://www.wi5.eu/

\bibitem{DCA-residential-2015} Y. Zhang, C. Jiang, Y. Wang, J. Yuan, and J. Cao, "United Channel Assignments in Residential Environments," in 2015 IEEE Global Communications Conference (GLOBECOM), 2015, pp. 1-6.

%\bibitem{DCA-802.11ac-2015} S. Jang and S. Bahk, "A Channel Allocation Algorithm for Reducing the Channel Sensing/Reserving Asymmetry in 802.11ac Networks," IEEE Transactions on Mobile Computing, vol. 14, no. 3, pp. 458-472, Mar. 2015.

%\bibitem{Ch-usage-based-2016} J. Nogueira and S. Sargento, "Channel Selection Relying on Probabilistic Adjacent Channel Interference Analysis and Pattern Recognition," Wireless Personal Communications, vol. 86, no. 3, pp. 1333-1357, Feb. 2016.

\bibitem{CA-VTC-14} B. A. H. S. Abeysekera, K. Ishihara, Y. Inoue, and M. Mizoguchi, "Network-Controlled Channel Allocation Scheme for IEEE 802.11 Wireless LANs: Experimental and Simulation Study," in 2014 IEEE 79th Vehicular Technology Conference (VTC Spring), 2014, pp. 1-5.

\bibitem{CA-BW-VTC-14} B. A. H. S. Abeysekera, M. Matsui, Y. Asai, and M. Mizoguchi, "Network controlled frequency channel and bandwidth allocation scheme for IEEE 802.11a/n/ac wireless LANs: RATOP," in 2014 IEEE 25th Annual International Symposium on Personal, Indoor, and Mobile Radio Communication (PIMRC), 2014, pp. 1041-1045.

%NEW papers
\bibitem{CAPWAP-based-CA-11} M. Bernaschi, F. Cacace, A. Davoli, D. Guerri, M. Latini, and L. Vollero, "A CAPWAP-based solution for frequency planning in large scale networks of WiFi Hot-Spots," Computer Communications, vol. 34, no. 11, pp. 1283-1293, Jul. 2011.

\bibitem{Measurement-CA-WCNC-10} Y. Liu, W. Wu, B. Wang, T. He, S. Yi, and Y. Xia, "Measurement-Based Channel Management in WLANs," in 2010 IEEE Wireless Communication and Networking Conference, 2010, pp. 1-6.

\bibitem{SDP} L. Vandenberghe, S. Boyd, Semidefinite programming, SIAM Review, vol. 38, no. 1, pp. 49-95, Mar. 1996.

\bibitem{CA-F-WCNC-11} H. Zhang, H. Ji, and W. Ge, "Channel assignment with fairness for multi-AP WLAN based on distributed coordination function," in 2011 IEEE Wireless Communications and Networking Conference, 2011, pp. 392-397.

\bibitem{Thr-estimation-2005} K.Duffy, D.Malone, and D.J.Leith, "Modeling the 802.1 distributed coordination function in non-saturated conditions", IEEE Communications Letters, Vol.9, No.8, pp.715-717, Aug.2005.

\bibitem {cvapPF} L. E. Li, M. Pal, and Y. R. Yang, "Proportional fairness in multi-rate wireless LANs," in Proc. IEEE INFOCOM,Apr. 2008, pp. 1004-1012.


\bibitem{802.11} IEEE Std 802.11-2007 (Revision of IEEE Std 802.11-1999), Jun. 2007.

\bibitem{SSF} I. Papanikos and M. Logothetis, "A study on dynamic load balance for IEEE 802.11b wireless LAN," In Proceedings of COMCON, Rethymna, Greece, 2001.

\bibitem{LLF} K. Sinha, S. C. Ghosh, B. P. Sinha, “Wireless Networks and Mobile Computing,” CRC Press, 2015.

\bibitem{MPD} J. C. Chen et. al., "Effective AP selection and load balancing in IEEE 802.11 wireless LANs," in Proc. IEEE Globecom, 2006.

\bibitem{Proxim} Proxim Wireless Networks. ORINOCO AP-600 data sheet, 2004.
\bibitem{CiscoADM} Cisco Systems Inc. Data sheet of Cisco Aironet 1200 series, 2004. 

\bibitem{F-LB-AsscCtrl-2004}Y. Bejerano, S.-J. Han, and L. (Erran) Li, "Fairness and Load Balancing in Wireless LANs Using Association Control," in Proceedings of the 10th Annual International Conference on Mobile Computing and Networking, 2004, pp. 315-329.


\bibitem{F-LB-AsscCtrl-2007} Y. Bejerano, S. J. Han, and L. Li, "Fairness and Load Balancing in Wireless LANs Using Association Control," IEEE/ACM Transactions on Networking, vol. 15, no. 3, pp. 560-573, Jun. 2007.


\bibitem{mob-Essex-2016} Y. Han and K. Yang, "An adaptive mobility manager for Software-Defined Enterprise WLANs," in 2016 Eighth International Conference on Ubiquitous and Future Networks (ICUFN), 2016, pp. 888-893.

\bibitem{802.11k} "IEEE Standard, Part 11: Wireless LAN Medium Access Control (MAC)and Physical Layer (PHY) Specifications Amendment 1: Radio
Resource Measurement of Wireless LANs," IEEE Std 802.11k-2008 (Amendment to IEEE Std 802.11-2007), pp. 1-244, June 2008.

\bibitem{Association-DenseWLANs-2014} A. Ozyagci, K. W. Sung, and J. Zander, "Association and Deployment Considerations in Dense Wireless LANs," in 2014 IEEE 79th Vehicular Technology Conference (VTC Spring), 2014, pp. 1-5.

\bibitem{DAM-G-3} D. Sajjadi, M. Tanha, and J. Pan, "Meta-Heuristic Solution for Dynamic Association Control in Virtualized Multi-Rate WLANs," in 2016 IEEE 41st Conference on Local Computer Networks (LCN), 2016, pp. 253-261.

\bibitem{DAM-G-4} G. S. Kasbekar, P. Nuggehalli, and J. Kuri, "Online Client-AP Association in WLANs," in 2006 4th International Symposium on Modeling and Optimization in Mobile, Ad Hoc and Wireless Networks, 2006, pp. 1-8.

\bibitem{DAM-G-5} D. Gong and Y. Yang, "AP association in 802.11n WLANs with heterogeneous clients," in 2012 Proceedings IEEE INFOCOM, 2012, pp. 1440-1448.

\bibitem{Association-CCA-2015} P. B. Oni and S. D. Blostein, "AP Association Optimization and CCA Threshold Adjustment in Dense WLANs," in 2015 IEEE Globecom Workshops (GC Wkshps), 2015, pp. 1-6.

\bibitem{Kuhn} G. A. Mills-Tettey, A. Stentz, and M. B. Dias, "The dynamic Hungarian algorithm for the assignment problem with changing costs," Robotics Institute, School of Computer Science, Carnegie Mellon University, PA, Tech. Rep. CMU-RI-TR-07-27, July 2007.

\bibitem{DAM-G-2} H. Gong and J. Kim, "Dynamic load balancing through association control of mobile users in WiFi networks," IEEE Transactions on Consumer Electronics, vol. 54, no. 2, pp. 342-348, May 2008.


\bibitem{802.11n-AP-Association-2014} D. Gong and Y. Yang, "On-Line AP Association Algorithms for 802.11n WLANs with Heterogeneous Clients," IEEE Transactions on Computers, vol. 63, no. 11, pp. 2772-2786, Nov. 2014.

\bibitem{BEST-AP} P. Dely et al., "BEST-AP: Non-intrusive estimation of available bandwidth and its application for dynamic access point selection," Computer Communications, vol. 39, pp. 78-91, Feb. 2014.

\bibitem{ChannelLoad} D. Gupta, D. Wu, P. Mohapatra, and C. N. Chuah, "Experimental Comparison of Bandwidth Estimation Tools for Wireless Mesh Networks," in IEEE INFOCOM 2009, 2009, pp. 2891-2895.


\bibitem{WBest} M. Li, M. Claypool, and R. Kinicki, "WBest: A bandwidth estimation tool for IEEE 802.11 wireless networks," in 2008 33rd IEEE Conference on Local Computer Networks (LCN), 2008, pp. 374-381.


\bibitem{Proportional-Fairness-AP-2014} W. Li et al., "AP Association for Proportional Fairness in Multirate WLANs," IEEE/ACM Transactions on Networking, vol. 22, no. 1, pp. 191-202, Feb. 2014.

\bibitem{Time-based-basic-1} M. Heusse, F. Rousseau, G. Berger-Sabbatel, and A. Duda, “Performance anomaly of 802.11b,” in IEEE INFOCOM 2003 - Twenty-second Annual Joint Conference of the IEEE Computer and Communications Societies, San Francisco, CA, USA, 2003, pp. 836-843.

\bibitem{Time-based-basic-2} G. Tan and J. Guttag, "Time-based Fairness Improves Performance in Multi-rate WLANs," in Proceedings of the Annual Conference on USENIX Annual Technical Conference, Berkeley, CA, USA, 2004, pp. 23-36.




\bibitem{DAM-G-1} H. Ko, J. Shin, D. Kwak, and C. Kim, "A joint approach to bandwidth allocation and AP-client association for WLANs," in IEEE Local Computer Network Conference, 2010, pp. 576-581.

\bibitem{Demand-aware-LB-Association-15} L. Yang, Y. Cui, H. Tang, and S. Xiao, "Demand-Aware Load Balancing in Wireless LANs Using Association Control," in 2015 IEEE Global Communications Conference (GLOBECOM), 2015, pp. 1-6.

\bibitem{Demand-aware-LB-Association-16-1} H. Tang, L. Yang, J. Dong, Z. Ou, Y. Cui, and J. Wu, "Throughput Optimization via Association Control in Wireless LANs," Mobile Netw Appl, vol. 21, no. 3, pp. 453-466, Jun. 2016.

\bibitem{NLB-13} F. Xu, X. Zhu, C. C. Tan, Q. Li, G. Yan, and J. Wu, "SmartAssoc: Decentralized Access Point Selection Algorithm to Improve Throughput," IEEE Transactions on Parallel and Distributed Systems, vol. 24, no. 12, pp. 2482-2491, Dec. 2013.

\bibitem{WiFiSeer} K. Sui et al., "Characterizing and Improving WiFi Latency in Large-Scale Operational Networks," in Proceedings of the 14th Annual International Conference on Mobile Systems, Applications, and Services, New York, NY, USA, 2016, pp. 347-360.

\bibitem{SNMP} S. Waldbusser, M. Rose, J. Case, and K. McCloghrie, "Protocol Operations for version 2 of the Simple Network Management Protocol (SNMPv2)." Available: https://tools.ietf.org/html/rfc1448.

\bibitem{random-forest} T. K. Ho, "Random decision forests," in Proceedings of 3rd International Conference on Document Analysis and Recognition, Montreal, QC, 1995, pp. 278-282.

\bibitem{flow-level-DAM} J. Chen, B. Liu, H. Zhou, Q. Yu, G. Lin, and X. Shen, "QoS-Driven Efficient Client Association in High-Density Software Defined WLAN," IEEE Transactions on Vehicular Technology, under press, 2017.

\bibitem{supermodular} G. Calinescu, C. Chekuri, M. P´al, and J. Vondr´ak, "Maximizing a submodular set function subject to a matroid constraint," in Integer programming and combinatorial optimization. Springer, 2007, pp. 182-196.

\bibitem{boundedAlg} X. Zhe, F. Zhang, W. Wang, and S. He, "A polynomial time algorithm for minimizing a nondecreasing supermodular set function and its performance guarantee," International Journal of Pure and Applied Mathematics, vol. 52, no. 5, pp. 637-643, 2009


\bibitem{Migration-DAM} W. Wong, A. Thakur, and S. H. G. Chan, "An approximation algorithm for AP association under user migration cost constraint," in IEEE INFOCOM 2016 - The 35th Annual IEEE International Conference on Computer Communications, 2016, pp. 1-9.

\bibitem{GameBased} L. H. Yen, J.-J. Li, and C.-M. Lin, "Stability and fairness of native AP selection games in IEEE 802.11 access networks," in 2010 Seventh International Conference on Wireless and Optical Communications Networks - (WOCN), 2010, pp. 1-5.

\bibitem{Jain's-fairness}  R. Jain,  D.M. Chiu and W. Hawe, "A Quantitative Measure of Fairness and Discrimination for Resource Allocation in Shared Computer Systems" DEC-Research Report TR-301, 1984.

\bibitem{Uplink-ref1}J. Oueis and E. C. Strinati, "Uplink Traffic in Future Mobile Networks: Pulling the Alarm," in Cognitive Radio Oriented Wireless Networks, 2016, pp. 583-593.

\bibitem{IOT-future1} I.-G. Lee and M. Kim, "Interference-aware self-optimizing Wi-Fi for high efficiency internet of things in dense networks," Computer Communications, vol. 89-90, pp. 60-74, Sep. 2016.

\bibitem{IOT-future2} K. Sood, S. Yu, and Y. Xiang, "Software-Defined Wireless Networking Opportunities and Challenges for Internet-of-Things: A Review," IEEE Internet of Things Journal, vol. 3, no. 4, pp. 453-463, Aug. 2016.

\bibitem{MARS} B. Dezfouli, M. Radi, and O. Chipara, “Mobility-aware real-time scheduling for low-power wireless networks,” in The 35th Annual IEEE International Conference on Computer Communications (INFOCOM), 2016, pp. 1–9.

\bibitem{RTwifi} Y.-H. Wei, Q. Leng, S. Han, A. K. Mok, W. Zhang, and M. Tomizuka, “RT-WiFi: Real-Time High-Speed Communication Protocol for Wireless Cyber-Physical Control Applications,” in IEEE 34th Real-Time Systems Symposium (RTSS), 2013, pp. 140–149.

\bibitem{CENTAUR} V. Shrivastava, N. Ahmed, S. Rayanchu, S. Banerjee, S. Keshav, K. Papagiannaki, and A. Mishra, “CENTAUR: Realizing the Full Potential of Centralized WLANs through a Hybrid Data Path,” in Proceedings of the 15th annual international conference on Mobile computing and networking - MobiCom ’09, 2009, p. 297.

%%%%Mobile data offloading: how much can WiFi deliver?
%%%%Per-node throughput enhancement in Wi-Fi DenseNets


%%%%%%% testbed-based performance evaluation papers
%%%%%\bibitem{single-BSS-testbed-2016} T. Zahid, F. Y. Dar, X. Hei, and W. Cheng, "A measurement study of a single-BSS software defined WiFi testbed," in 2016 First IEEE International Conference on Computer Communication and the Internet (ICCCI), 2016, pp. 144-147.
%%%%%\bibitem{multi-BSS-testbed-2016} T. Zahid, X. Hei, and W. Cheng, "Understanding performance bottlenecks of a multi-BSS software defined WiFi network testbed," in 2016 First IEEE International Conference on Computer Communication and the Internet (ICCCI), 2016, pp. 153-156.
%%%%%
%%%%%
%%%%%
%%%%%
%%%%%%2
%%%%%\bibitem{MWO-1} S. Srikanteswara, G. Li, and C. Maciocco, "Cross Layer Interference Mitigation Using Spectrum Sensing," in IEEE GLOBECOM 2007 - IEEE Global Telecommunications Conference, 2007, pp. 3553-3557.
%%%%%%3
%%%%%\bibitem{MWO-2} G. Li, S. Srikanteswara, and C. Maciocco, "Spectrum-sensing based interference mitigation for WLAN devices," in 3rd International Conference on Communication Systems Software and Middleware and Workshops, 2008. COMSWARE 2008, 2008, pp. 402-408.
%%%%%%4
%%%%%\bibitem{MBSA-TDL} A. Z. Al-Banna, J. L. LoCicero, and D. R. Ucci, "Multi-Element Adaptive Arrays with Tapped Delay Lines for Interference Mitigation in IEEE 802.11G OFDM Systems," in MILCOM 2007 - IEEE Military Communications Conference, 2007, pp. 1-8.
%%%%%%5
%%%%%\bibitem{power-ctrl-1} V. P. Mhatre, K. Papagiannaki, and F. Baccelli, "Interference Mitigation Through Power Control in High Density 802.11 WLANs," in IEEE INFOCOM 2007 - 26th IEEE International Conference on Computer Communications, 2007, pp. 535-543.
%%%%%%6
%%%%%\bibitem{CRRM-1} S. J. Bae, B. G. Choi, H. S. Chae, and M. Y. Chung, "Self-configuration scheme to alleviate interference among APs in IEEE 802.11 WLAN," in 2012 IEEE 23rd International Symposium on Personal, Indoor and Mobile Radio Communications - (PIMRC), 2012, pp. 1025-1030.
%%%%%%7
%%%%%\bibitem{DenseNets-survey} K. Shin, I. Park, J. Hong, D. Har, and D. h Cho, "Per-node throughput enhancement in Wi-Fi densenets," IEEE Communications Magazine, vol. 53, no. 1, pp. 118-125, Jan. 2015.
%%%%%%8
%%%%%\bibitem{VOID} K. Cai, M. Blackstock, M. J. Feeley, and C. Krasic, "Non-intrusive, Dynamic Interference Detection for 802.11 Networks," in Proceedings of the 9th ACM SIGCOMM Conference on Internet Measurement Conference, New York, NY, USA, 2009, pp. 377-383.
%%%%%%book 
%%%%%\bibitem{MLR-book} D. A. Freedman, Statistical Models: Theory and Practice, 2 edition. Cambridge ; New York: Cambridge University Press, 2009.
%%%%%%9
%%%%%\bibitem{Mitigation-1} N. Ahmed, V. Shrivastava, A. Mishra, S. Banerjee, S. Keshav, and K. Papagiannaki, "Interference Mitigation in Enterprise WLANs Through Speculative Scheduling," in Proceedings of the 13th Annual ACM International Conference on Mobile Computing and Networking, New York, NY, USA, 2007, pp. 342-345.
%%%%%%10
%%%%%\bibitem{Mitigation-2} M. Abusubaih, B. Rathke, and A. Wolisz, "A framework for interference mitigation in multi-BSS 802.11 wireless LANs," in World of Wireless, Mobile and Multimedia Networks Workshops, IEEE WoWMoM 2009, pp. 1-11.
%%%%%%10
%%%%%\bibitem{optimal-design} V. P. Mhatre and K. Papagiannaki, "Optimal Design of High Density 802.11 WLANs," in Proceedings of the 2006 ACM CoNEXT Conference, New York, NY, USA, 2006, p. 8:1-8:12.
%%%%%% citations of 5
%%%%%\bibitem{symphony} K. Ramachandran, R. Kokku, H. Zhang, and M. Gruteser, "Symphony: Synchronous Two-Phase Rate and Power Control in 802.11 WLANs," IEEE/ACM Transactions on Networking, vol. 18, no. 4, pp. 1289-1302, Aug. 2010.
%%%%%
%%%%%\bibitem{symphony-29} "Multiband Atheros driver for WiFi," MadWifi [Online]. Available: http:$//$www.madwifi.org.
%%%%%
%%%%%\bibitem{symphony-41} D. Raychaudhuri, I. Seskar, M. Ott, S. Ganu, K. Ramachandran, H. Kremo, R. Siracusa, H. Liu, and M. Singh, "Overview of the ORBIT radio grid testbed for evaluation of next-generation wireless network protocols," in Proc. IEEE WCNC, Mar. 2005, vol. 3, pp. 1664-1669.
%%%%%
%%%%%\bibitem{MinPACK} W. Wang, Q. Wang, W. K. Leong, B. Leong, and Y. Li, "Uncovering a Hidden wireless menace: Interference from 802.11x MAC acknowledgment frames," in 2014 Eleventh Annual IEEE International Conference on Sensing, Communication, and Networking (SECON), 2014, pp. 117-125.
%%%%%
%%%%%
%%%%%
%%%%%\begin{itemize}
%%%%%\item \textcolor{blue}{\textbf{Papers on 
 %}}
%%%%%\end{itemize}
%%%%%%%%%%
%%%%%\bibitem{ac-27} B. Bellalta, A. Checco, A. Zocca, and J. Barcelo, "On the Interactions Between Multiple Overlapping WLANs Using Channel Bonding," IEEE Transactions on Vehicular Technology, vol. 65, no. 2, pp. 796-812, Feb. 2016.
%%%%%\bibitem{ac-48} W.-S. Jung, K.-W. Lim, and Y.-B. Ko, "Utilising partially overlapped channels for OFDM-based 802.11 WLANs," Computer Communications, vol. 63, pp. 77-86, Jun. 2015.
%%%%%\bibitem{ac-41} Q. Wang, L. J. Greenstein, L. J. Cimini, D. S. Chan, and A. Hedayat, "Multi-User and Single-User Throughputs for Downlink MIMO Channels with Outdated Channel State Information," IEEE Wireless Communications Letters, vol. 3, no. 3, pp. 321-324, Jun. 2014.
%%%%%\bibitem{ac-34} Y. Zeng, P. H. Pathak, and P. Mohapatra, "A first look at 802.11ac in action: Energy efficiency and interference characterization," in Networking Conference, 2014 IFIP, 2014, pp. 1-9.
%%%%%\bibitem{ac-38} M. Yazid, A. Ksentini, L. Bouallouche-Medjkoune, and D. Aissani, "Performance Analysis of the TXOP Sharing Mechanism in the VHT IEEE 802.11ac WLANs," IEEE Communications Letters, vol. 18, no. 9, pp. 1599-1602, Sep. 2014.
%%%%%\bibitem{ac-37} O. Sharon and Y. Alpert, "MAC level Throughput comparison: 802.11ac vs. 802.11n," Physical Communication, vol. 12, pp. 33-49, Sep. 2014.
%%%%%%\bibitem{ac-40} O. Bejarano, E. Magistretti, O. Gurewitz, and E. W. Knightly, "MUTE: Sounding inhibition for MU-MIMO WLANs," in 2014 Eleventh Annual IEEE International Conference on Sensing, Communication, and Networking (SECON), 2014, pp. 135-143.
%%%%%\bibitem{ac-46}C. Zhu, C. Ngo, A. Bhatt, and Y. Kim, "Enhancing WLAN backoff procedures for downlink MU-MIMO support," in 2013 IEEE Wireless Communications and Networking Conference (WCNC), 2013, pp. 368-373.







\end{thebibliography}


==> table-comp-jay.tex <==
        
        
        DenseAP \cite{DenseAP}&$\times$&$\times$&$\times$&$\times$&Proprietary&$\times$& $\times$ &$\checkmark$&$\times$\\\hline
        % SB X + Y    NB: Z
		CUWN \cite{Cisco}&$\times$&$\times$&$\times$&$\times$&CAPWAP&$\checkmark$&$\times$&$\checkmark$&$\checkmark$\\\hline

		DIRAC \cite{DIRAC} &$\checkmark$&$\checkmark$&$\times$&$\times$& Proprietary &$\times$& $\times$ &$\checkmark$&$\times$\\\hline
		
		Trantor \cite{Trantor}&\textbf{$\checkmark$}&$\checkmark$&$\times$&$\times$&Proprietary&$\times$&$\checkmark$&$\times$&$\times$\\\hline
		%
		%		
		Dyson \cite{Dyson}&$\checkmark$&$\checkmark$&$\times$&$\times$&Proprietary&$\times$&$\checkmark$&$\checkmark$&$\times$\\\hline
		%		
		$\AE$therFlow  \cite{AEtherFlow}&$\checkmark$&$\checkmark$&$\times$&$\times$& Extended OpenFlow  &$\times$&$\times$&$\checkmark$&$\times$\\\hline		
        %
		WVT \cite{smith2007wireless}&$\times$&$\times$&$\checkmark$& $\checkmark$ & Proprietary &$\times$&$\times$&$\times$&$\times$\\\hline
        %        
		AP Aggregate \cite{nagai2011framework}&$\times$&$\times$&$\checkmark$& $\checkmark$ & Proprietary &$\times$&$\times$&$\checkmark$&$\times$\\\hline
        %        
		%
		Odin \cite{Odin,Odin2,OdinThor}&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$& OpenFlow+Proprietary &$\checkmark$&$\times$&$\checkmark$&$\times$\\\hline
        %
		SplitAP \cite{SplitAP}&$\times$&$\times$&$\checkmark$&$\checkmark$& Proprietary &$\times$&$\checkmark$&$\times$&$\times$\\\hline		
		%
		CloudMAC \cite{CloudMAC,CloudMAC3}&$\checkmark$&$\times$&$\checkmark$&$\checkmark$& OpenFlow &$\checkmark$&$\times$&$\checkmark$&$\checkmark$\\\hline				
		%
		EmPOWER \cite{EmPOWER}&$\checkmark$&$\times$&$\checkmark$&$\times$& OpenFlow+REST &$\checkmark$&$\times$&$\checkmark$&$\times$\\\hline		
		%
		%
		EmPOWER2 \cite{Primitives}&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$& OpenFlow &$\checkmark$&$\times$&$\checkmark$&$\checkmark$\\\hline				
		%
		Sd-wlan \cite{SDWLAN}&$\checkmark$&$\times$&$\checkmark$&$\times$& Extended OpenFlow &$\checkmark$&$\times$&$\checkmark$&$\times$\\\hline
        %		
		BeHop \cite{BeHop}&$\checkmark$&$\times$&$\checkmark$&$\times$& OpenFlow+Proprietary &$\checkmark$&$\times$&$\times$&$\times$\\\hline
		%		% a configuration API for channel and power allocation --> No details about API !!!
		%
		RCWLAN \cite{nakauchi2012airtime}&$\times$&$\times$&$\checkmark$&$\checkmark$& Proprietary &$\times$&$\times$&$\times$&$\times$\\\hline	
        %		
		vBS \cite{vBS}&$\checkmark$&$\times$&$\checkmark$&$\checkmark$& OpenFlow &$\times$&$\times$&$\checkmark$&$\times$\\\hline				
        %        
		BIGAP \cite{BIGAP}&$\checkmark$&$\checkmark$&$\checkmark$&$\times$& Proprietary &$\times$&$\times$&$\checkmark$&$\checkmark$\\\hline		
        %        
		AeroFlux \cite{AeroFlux}&$\checkmark$&$\checkmark$&$\checkmark$&$\times$& Extended OpenFlow &$\checkmark$&$\times$&$\checkmark$&$\times$\\\hline		
        %        
		Ethanol \cite{Ethanol}&$\checkmark$&$\checkmark$&$\checkmark$&$\times$& OpenFlow+Proprietary &$\checkmark$&$\times$&$\checkmark$&$\times$\\\hline
        %        
		OpenSDWN \cite{OpenSDWN}&$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$& OpenFlow+Proprietary  &$\checkmark$&$\times$&$\checkmark$&$\times$\\\hline
        %        
		VAN \cite{VAN} &$\checkmark$&$\checkmark$&$\times$&$\checkmark$& OpenFlow &$\times$&$\times$&$\times$&$\times$\\\hline	
		%		%		
		%		
		COAP \cite{COAP}&$\checkmark$&$\checkmark$&$\times$&$\times$& OpenFlow+Proprietary  &$\times$&$\times$&$\times$&$\checkmark$\\\hline
		%		
		%		%		%
		%
		%		%
		ResFi \cite{ResFi}&$\checkmark$&$\checkmark$&$\checkmark$&$\times$& Proprietary &$\times$&$\times$&$\checkmark$&$\checkmark$\\\Xhline{3\arrayrulewidth}	
